Save the Farms: Nonlinear Impact of Climate Change on Banks' Agricultural Lending

The agricultural sector is particularly susceptible to the impact of climate change. In this paper, I investigate how vulnerability to climate change affects U.S. farms' credit access, and demonstrates that such impact is unequally distributed across farms. I first construct a theoretical framework of bank lending to farms faced with climate risks, and the model helps discipline ensuing empirical analyses that use novel panel datasets at county and at bank levels. I find that higher exposure to climate change, measured by temperature anomaly, reduces bank lending to farms. Such impact is persistent, nonlinear, and heterogeneous. Small and medium farms almost always experience loss of loan access. In comparison, large farms see less severe credit contraction, and in some cases may even see improvement in funding. While small banks carry the burden of continuing to lend to small farms, their limited market share cannot compensate for the reduction of lending from medium and large banks. These results suggest that factors such as farm size and bank type can amplify the financial impact of climate change.

==> tables/table1_n.tex <==
\begin{tabular}{lcccc} \hline
 & (1) & (2) & (3) & (4) \\
VARIABLES & Num. to large farms & Amount to large farms & Num. to small-mid farms & Amount to small-mid farms \\ \hline
 &  &  &  &  \\
Coastal Storm & 1.66** & 29.74 & 0.12 & -84.12 \\
 & (0.73) & (52.88) & (1.91) & (122.65) \\
Flood & -0.81*** & -28.47 & -1.72** & -82.59* \\
 & (0.30) & (25.15) & (0.80) & (48.62) \\
Freezing (lagged) & 10.56 & 441.99* & 7.40 & 430.75 \\
 & (8.45) & (245.89) & (8.50) & (278.70) \\
Hurricane & -0.91*** & -37.13*** & -0.59* & -76.82*** \\
 & (0.15) & (8.62) & (0.31) & (17.10) \\
Landslide & -8.14*** & -406.09** & 8.48*** & -112.70 \\
 & (1.77) & (162.98) & (3.11) & (129.14) \\
Ice storm (lagged) & -0.78*** & -42.75*** & 1.48 & 64.65 \\
 & (0.22) & (16.05) & (0.96) & (46.40) \\
Storm & -0.32** & -29.53*** & -1.51*** & -54.64** \\
 & (0.12) & (10.19) & (0.44) & (22.74) \\
Snow (lagged) & -0.02 & -30.26 & -5.66*** & -122.69** \\
 & (0.24) & (22.72) & (0.96) & (55.23) \\
Tornado & -1.14* & 20.95 & 3.60 & 294.29* \\
 & (0.67) & (66.38) & (2.78) & (156.99) \\
 &  &  &  &  \\
Observations & 69,728 & 69,728 & 69,728 & 69,728 \\
R-squared & 0.204 & 0.094 & 0.141 & 0.059 \\
County FE & Yes & Yes & Yes & Yes \\
Year FE & Yes & Yes & Yes & Yes \\
Region x Year FE & Yes & Yes & Yes & Yes \\
 Robust SE & Cluster & Cluster & Cluster & Cluster \\ \hline
\multicolumn{5}{c}{ Robust standard errors in parentheses} \\
\multicolumn{5}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}


==> tables/table3_r.tex <==
\begin{tabular}{lcccc} \hline
 & (1) & (2) & (3) & (4) \\
VARIABLES & Num. to large farms & Amount to large farms & Num. to small-mid farms & Amount to small-mid farms \\ \hline
 &  &  &  &  \\
High temperature anomaly & -0.09 & 5.13 & 1.34*** & 115.41*** \\
 & (0.09) & (7.40) & (0.20) & (16.96) \\
High temperature anomaly (square) & 0.02 & -1.17 & -0.85*** & -49.73*** \\
 & (0.03) & (2.35) & (0.08) & (5.46) \\
Precipitation anomaly & 0.24** & 36.89*** & -0.76** & 27.22 \\
 & (0.12) & (10.23) & (0.34) & (25.39) \\
Precipitation anomaly (square) & -0.11 & 24.90*** & -0.63*** & 50.60** \\
 & (0.08) & (6.96) & (0.22) & (19.87) \\
 &  &  &  &  \\
Observations & 72,834 & 72,834 & 72,834 & 72,834 \\
R-squared & 0.193 & 0.050 & 0.133 & 0.104 \\
County FE & Yes & Yes & Yes & Yes \\
Year FE & Yes & Yes & Yes & Yes \\
Region x Year FE & Yes & Yes & Yes & Yes \\
 Robust SE & Cluster & Cluster & Cluster & Cluster \\ \hline
\multicolumn{5}{c}{ Robust standard errors in parentheses} \\
\multicolumn{5}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}


==> tables/table4new.tex <==
\begin{tabular}{lcccc} \hline
 & (1) & (2) & (3) & (4) \\
VARIABLES & Num. to large farms & Amount to large farms & Num. to small-mid farms & Amount to small-mid farms \\ \hline
 &  &  &  &  \\
High temperature anomaly & -0.14* & -1.96 & 1.48*** & 111.01*** \\
 & (0.08) & (7.10) & (0.19) & (15.62) \\
High temperature anomaly (square) & 0.01 & -1.08 & -0.85*** & -48.80*** \\
 & (0.03) & (2.35) & (0.07) & (5.42) \\
 &  &  &  &  \\
Observations & 72,834 & 72,834 & 72,834 & 72,834 \\
R-squared & 0.194 & 0.050 & 0.134 & 0.105 \\
County FE & Yes & Yes & Yes & Yes \\
Year FE & Yes & Yes & Yes & Yes \\
Region x Year FE & Yes & Yes & Yes & Yes \\
 Robust SE & Cluster & Cluster & Cluster & Cluster \\ \hline
\multicolumn{5}{c}{ Robust standard errors in parentheses} \\
\multicolumn{5}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}


==> tables/table5.tex <==
\begin{tabular}{lcccc} \hline
 & (1) & (2) & (3) & (4) \\
VARIABLES & Num. to large farms & Amount to large farms & Num. to small-mid farms & Amount to small-mid farms \\ \hline
 &  &  &  &  \\
High temperature anomaly & -0.14* & -10.11 & 1.55*** & 57.36*** \\
 & (0.08) & (6.18) & (0.19) & (12.05) \\
High temperature anomaly (square) & 0.02 & 1.99 & -0.85*** & -27.87*** \\
 & (0.03) & (2.06) & (0.08) & (4.37) \\
Total number of bank branches & 0.21*** & 0.16 & 0.22*** & 2.47 \\
 & (0.02) & (1.60) & (0.04) & (1.89) \\
Temp. anomaly x Bank Branches & -0.01 & -0.69 & -0.02 & -0.74 \\
 & (0.01) & (0.50) & (0.03) & (0.52) \\
Temp. anomaly (square) x Bank Branches & -0.01*** & 0.40 & -0.03*** & 0.08 \\
 & (0.00) & (0.36) & (0.01) & (0.37) \\
 &  &  &  &  \\
Observations & 72,447 & 72,447 & 72,447 & 72,447 \\
R-squared & 0.204 & 0.094 & 0.134 & 0.056 \\
County FE & Yes & Yes & Yes & Yes \\
Year FE & Yes & Yes & Yes & Yes \\
Region x Year FE & Yes & Yes & Yes & Yes \\
 Robust SE & Cluster & Cluster & Cluster & Cluster \\ \hline
\multicolumn{5}{c}{ Robust standard errors in parentheses} \\
\multicolumn{5}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}

